Murmurations of Hecke $L$-Functions of Imaginary Quadratic Fields

We calculate the murmuration density for the family of Hecke $L$-functions of imaginary quadratic fields associated to non-trivial characters. This density exhibits a universality property like Zubrilina's density for the murmurations of holomorphic modular forms. We show all murmuration functions obtained by averaging over the family with a compactly supported smooth weight function has asymptotics compatible with the 1-level density conjecture of Katz and Sarnak. The novelty of the murmurations of this family of $L$-functions is its pronounced almost periodic feature, which allows one to describe this murmuration without averaging over primes, and which is non-existent or previously unnoticed for other families.

==> sections/A.2_on_GRH.tex <==
% \newpage
\subsection{Error Bounds Assuming GRH}\label{section:errors_on_GRH}
In this section we compute the error bounds for Theorem \ref{thm:thm1} assuming the Generalized Riemann Hypothesis, therefore justifying the remark after the Theorem. The change is that we can now apply Corollary \ref{cor:truncation_assuming_GRH} in place of Lemma \ref{lem:density_theorem} when truncating $L$-functions. This gives better (and aesthetically more pleasing, frankly) error bounds.

In Section \ref{section:denom_and_num_minus}, we have $$\Err_1\ll\left(T^{-1/2}X^{1/2}Y+X^{-1/2}Y^2+Y\right)(TX)^\epsilon$$ in place of \ref{eqn:section_2_error}. The total error for $G_{\denom}$ is $$\Err\ll\left(T^{1/5}X^{11/10}+T^{-1/2}X^{1/2}Y+X^{-1/2}Y^2+Y\right)(TX)^\epsilon\ll\left(X^{-1/2}Y^2+X^{13/14}Y^{2/7}\right)(XY)^\epsilon$$ upon choosing $T=X^{-6/7}Y^{10/7}$. Consequently, we have $$G_{\denom}^{-1}=\frac{11\pi\zeta(2)}{4A}\frac{1}{Y\sqrt{X}}+O\left(\left(X^{-3/2}+X^{-1/14}Y^{-12/7}\right)(XY)^\epsilon\right)$$ in place of \ref{eqn:G_denom_inverse}.

In Chapter \ref{section:contribution_y=1}, we have $$\Err_2\ll\left(T^{-1/2}X^{1/2}Y+X^{-1/2}Y^2\right)(TX)^\epsilon$$ in place of \ref{eqn:Err_2}. The other terms in \ref{eqn:Err_cumulative_Theorem_3.1} are unchanged, so the error for Theorem \ref{thm:thm_y=1} is \begin{align*}
    \Err&\ll_{\delta_\xi}\begin{multlined}[t]
        \Bigg(T^{1/2}Vp^{1/2}X^{1/2}+\frac{X^{1/2}Y}{T^{1/2}}+\frac{X^{1/2}Y}{V}+\frac{p^{7/6}X^{1/2}}{V^{2/3}}+\frac{p^{3/2}X^{1/2}}{V^2}+p^{5/6}X^{1/2}\\+\frac{X^{1/2}Y}{T^{1/2}}+\frac{Y^2}{X^{1/2}}+\frac{X^{1/2}Y^2}{p}\Bigg)(TVpXY)^\epsilon
    \end{multlined}\\
    &\ll\left(p^{9/10}X^{1/2}Y^{1/35}+\frac{Y^2}{X^{1/2}}\right)(pXY)^\epsilon
\end{align*} upon choosing $S=p^{2/5}Y^{-3/70},T=Y^{1/7}$. This is carried to Theorem \ref{thm:thm_y=y} with an extra factor of $y^{2+\epsilon}$ as usual.

Putting it together, the error for Theorem \ref{thm:thm1} under GRH is \begin{align*}
    \Err&\ll_{\delta_\xi}\begin{multlined}[t]
        \frac{1}{Y\sqrt{X}}\left[\frac{p}{X}\left(p^{9/10}X^{1/2}Y^{1/35}+\frac{Y^2}{X^{1/2}}\right)(pXY)^\epsilon+p^{7/10+\epsilon}X^{3/5+\epsilon}+p^{1+\epsilon}\right]\\+Y\sqrt{p}\left[\left(X^{-3/2}+X^{-1/14}Y^{-12/7}\right)(XY)^\epsilon\right]
    \end{multlined}\\
    &\ll\left(\frac{p^{19/10}}{XY^{34/35}}+\frac{pY}{X^2}\right)(pXY)^\epsilon.
\end{align*} This is $O\left(X^{-\delta_0+\epsilon}\right)$ with $$\delta_0=\min\left\{\frac{1}{14}-\frac{34}{35}\delta_Y-\frac{19}{10}\delta_p,\delta_Y-\delta_p\right\},$$ as claimed in the remark after Theorem \ref{thm:thm1}.
